The Competition for Partners in Matching Markets

We study the competition for partners in two-sided matching markets with heterogeneous agent preferences, with a focus on how the equilibrium outcomes depend on the connectivity in the market. We model random partially connected markets, with each agent having an average degree $d$ in a random (undirected) graph, and a uniformly random preference ranking over their neighbors in the graph. We formally characterize stable matchings in large markets random with small imbalance and find a threshold in the connectivity $d$ at $\log^2 n$ (where $n$ is the number of agents on one side of the market) which separates a ``weak competition'' regime, where agents on both sides of the market do equally well, from a ``strong competition'' regime, where agents on the short (long) side of the market enjoy a significant advantage (disadvantage). Numerical simulations confirm and sharpen our theoretical predictions, and demonstrate robustness to our assumptions. We leverage our characterizations in two ways: First, we derive prescriptive insights into how to design the connectivity of the market to trade off optimally between the average agent welfare achieved and the number of agents who remain unmatched in the market. For most market primitives, we find that the optimal connectivity should lie in the weak competition regime or at the threshold between the regimes. Second, our analysis uncovers a new conceptual principle governing whether the short side enjoys a significant advantage in a given matching market, which can moreover be applied as a diagnostic tool given only basic summary statistics for the market. Counterfactual analyses using data on centralized high school admissions in a major USA city show the practical value of both our design insights and our diagnostic principle.

==> conclusion.tex <==
We did a very great job.

==> lemma-upper-bound-on-unmatched-women.tex <==
\begin{lemma}
Consider the setting of Theorem~\ref{thm:main-result}. For large enough $n$, we have the following upper bound on the expected number of unmatched women under stable matching
\begin{align}
  \Ex [\delta^w] \leq n \exp(-\sqrt{d} + 1.5d^{1/4}) \, .
\end{align}
\end{lemma}

\begin{proof}
We will track the progress of the man proposing DA algorithm making use of the principle of deferred decisions, and further make use of a particular sequence of proposals: we will specify beforehand an arbitrary man $i$ (before any information whatsoever is revealed), and then run DA to convergence on the other men, before man $i$ makes a single proposal.  We will show that the probability that the man $i$ remains unmatched is bounded as
\begin{align}
\prob(\mu(i) = i) \leq \exp(-\sqrt{d} + 1.4d^{1/4})
\label{eq:prob-i-unmatched-ub}
\end{align}
for large enough $n$.
This will imply that, by symmetry across men, the expected number of unmatched men under stable matching will be bounded above as
$$\Ex[\delta^m] \leq  (n+k)\exp(-\sqrt{d} + 1.4 d^{1/4})\, .$$
Finally the number of unmatched women at the end is exactly $\delta^w = \delta^m -k$, and so
$$\Ex[\delta^w] = \Ex[\delta^m] -k \leq (n+k)\exp(-\sqrt{d} + 1.4d^{1/4}) - k \leq n \exp(-\sqrt{d} + 1.5d^{1/4})$$ for large enough $n$
as required, using $k = O(ne^{-\sqrt{d}})$. The rest of proof is devoted to establishing \eqref{eq:prob-i-unmatched-ub}.

%Let the number of proposals made up to the point where DA converges on the men besides $i$ (whereas $i$ has yet to make a proposal) be $\tau'$ and let the number of unmatched women at that point be $\delta^w(\tau')$.
%As a preliminary observation, note that at the end of DA, we must have $\tau \geq \tau'$ (the number of proposals will increase from here) and $\delta^w \leq \delta^w(\tau')$ (the number of unmatched women will either remain the same or decrease (by one, in fact)). Hence, u
Using Lemma~\ref{lem:total-proposal-upper-bound}, we have that with probability $1 - O(\exp(-\sqrt{n}))$, at the end of DA, $\tau$ is bounded above as
	\begin{align}
	\tau
		\leq n \big (
		\sqrt{d}
		+
		d^{\frac{1}{4}} \big )
		\, ,
\label{eq:tauprime-ub}
	\end{align}
and using Lemma~\ref{lem:unmatched-women-lower-bound}, we have that with probability $1 - O(\exp(-\sqrt{n}))$, we have
	\begin{align}
\delta^w \geq ne^{-\sqrt{d} - 2 d^{\frac{1}{4}}}
	\, .
\label{eq:deltaprime-lb}
	\end{align}
at the end of DA. Note that if \eqref{eq:tauprime-ub} holds at the end of DA, then the RHS is an upper bound on $t$ throughout the run of DA. Similarly, since the number of unmatched woman $\delta^w[t]$ is monotone non-increasing in $t$, if \eqref{eq:deltaprime-lb} holds at the end of DA, then the RHS of \eqref{eq:deltaprime-lb} is a lower bound on $\delta^w[t]$ throughout the run of DA.
%\edit{Furthermore, from Lemma ????, with probability $1 - O(\exp(-\sqrt{n}))$, no individual woman receives more than $\sqrt{n}$ proposals during man proposing DA,
%\begin{align}
%w_{i, \tau} \leq \sqrt{n} \qquad \forall i \in \cW\, .
%\label{eq:womens-rank-ub}
%\end{align}}
If, at any stage during the run of DA either \eqref{eq:tauprime-ub} (with $t$ instead of $\tau$) or \eqref{eq:deltaprime-lb} (with $\delta^w[t]$ instead of $\delta^w$) % or \eqref{eq:womens-rank-ub}
is violated, declare a ``failure'' event $\Ev \equiv \Ev_\tau$. By union bound, we know that $\prob(\Ev) = O(\exp(-\sqrt{n}))$. For $t \leq \tau$, let $\Ev_t$ denote the event that no failure has occurred during the first $t$ proposals of DA. We will prove \eqref{eq:prob-i-unmatched-ub} by showing an upper bound on the likelihood that man $i$ remains unmatched for sample paths where no failure occurs, and assuming the worst (i.e., that $i$ certainly remains unmatched) in the rare cases where there is a failure.

Run DA to convergence on men besides $i$. Now consider proposals by $i$. At each such proposal, the recipient woman is drawn uniformly at random from among at least $n - d+ 1$ ``candidate''  women (the ones to whom $i$ has not yet proposed). Assuming $\Ev_t^c$, we know that
	\begin{align}
	t\leq n \big (\sqrt{d} + d^{\frac{1}{4}} \big )\, ,
\label{eq:t-ub}
	\end{align}
and hence the total number of proposals received by candidate women is at most $ n \big (\sqrt{d} + d^{\frac{1}{4}} \big )$, and hence the average number of proposals received by candidate women is at most \edit{$n(\sqrt{d}	+ d^{\frac{1}{4}})/(n-d+1) \leq \sqrt{d}(1	+ d^{-1/4} + \log^2 n/n) \leq \sqrt{d}(1	+ 1.1d^{-\frac{1}{4}}) \leq \sqrt{d} + 1.1d^{\frac{1}{4}}$ for large enough $n$, using $d = o(\log^2 n)$}. If the proposal goes to woman $j$, the probability of it being accepted is
$\frac{1}{w_{j,t}+1}$. Averaging over the candidate women and using Jensen's inequality for the function $f(x) = \frac{1}{x+1}$, the probability of the proposal being accepted is at least $\frac{1}{\sqrt{d} + 1.1d^{1/4}+1} \geq \frac{1}{\sqrt{d} + 1.2d^{1/4}}$. If the proposal is accepted, say by woman $j$, this triggers a rejection chain. We show that it is very unlikely that this rejection chain will cause an additional proposal to woman $j$ (which will imply that it is very unlikely that the rejection chain will cause $i$ himself to be rejected): For every additional proposal in the rejection chain, the likelihood that it goes to  an unmatched woman far exceeds the likelihood that it goes to woman $j$: if the current time is $t'$ and $\Ev_{t'}^c$ holds, then, since all $\delta^w[t']$ unmatched women are certainly candidate recipients of the next proposal, the likelihood of the proposal being to an unmatched woman is at least $\delta^w[t'] \geq ne^{-\sqrt{d} - 2 d^{\frac{1}{4}}} \geq \sqrt{n}$ times the likelihood of it being to woman $j$ for $n$ large enough, using $d = o(\log^2 n)$. Now if the proposal is to an unmatched woman, this causes the rejection chain to terminate, hence the expected number of proposals to an unmatched woman in the rejection chain is at most $1$. We immediately deduce that if a failure does not occur prior to termination of the chain, the expected number of proposals to woman $j$ in the rejection chain is at most $\frac{1}{\sqrt{n}}$. It follows that
\begin{align*}
  &  \prob(i \textup{ is displaced from $j$ by the rejection chain triggered when $j$ accepts his proposal}) \\
  \leq \; & \prob(j \textup{ receives a proposal in the rejection chain triggered}) \\
  \leq \; & \Ex [\textup{Number of proposals received by $j$ in the rejection chain triggered}]\\
  \leq \; &  \frac{1}{\sqrt{n}} \, ,
\end{align*}
for $n$ large enough.
Overall, the probability of the proposal by $i$ being ``successful'' in that it is both (a) accepted, and then (b) man $i$ is not pushed out by the rejection chain, is at least
\begin{align*}
\frac{1}{\sqrt{d} + 1.2d^{1/4}} \left ( 1- \frac{1}{\sqrt{n}} \right )
\leq \frac{1}{\sqrt{d} + 1.3d^{1/4}}\, ,
\end{align*}
for large enough $n$. Hence the probability of an unsuccessful proposal (if there is no failure) is at most
\begin{align*}
1- \frac{1}{\sqrt{d} + 1.3d^{1/4}} \leq \exp\left \{ - \frac{1}{\sqrt{d} + 1.3d^{1/4}} \right \} \, ,
\end{align*}
and so the probability of all $d$ proposals being unsuccessful (if there is no failure) is at most
\begin{align*}
  \exp\left \{ - \frac{d}{\sqrt{d} + 1.3d^{1/4}} \right \} \leq \exp \left \{ - \sqrt{d} + 1.3 d^{1/4}\right \} \, .
\end{align*}
Formally, what we have obtained is an upper bound on the quantity $\Ex\big [ \ind(\mu(i) = i)\ind(\Ev^c)\big ]$, namely, 
\begin{align*}
\Ex\big [ \ind(\mu(i) = i)\ind(\Ev^c)\big ] \leq \exp \left \{ - \sqrt{d} + 1.3 d^{1/4}\right \}\, .
\end{align*} 

Since the probability of failure is bounded as $\prob(\Ev) \leq O(\exp(-\sqrt{n}))$, the overall probability that of man $i$ remaining unmatched is bounded above as
\begin{align*}
  \prob(\mu(i) = i) &\leq \Ex\big [ \ind(\mu(i) = i) \ind(\Ev^c)\big ] + \prob(\Ev)\\
  &\leq  \exp \left \{ - \sqrt{d} + 1.3 d^{1/4}\right \}  + O(\exp(-\sqrt{n})) \leq \exp \left \{ - \sqrt{d} + 1.4 d^{1/4}\right \}\,
\end{align*}
for large enough $n$, i.e., the bound \eqref{eq:prob-i-unmatched-ub} which we set out to show.
%\yk{In progress.}
%A union bound immediately tells us that with probability $1 - O(\exp(-\sqrt{n}))$, the bounds in \eqref{eq:tauprime-ub} and \eqref{eq:deltaprime-lb} \emph{both} hold. Suppose this is the case. Now consider a proposal by man $i$. The proposal is to a uniformly random woman to whom $i$ has not yet proposed. There are at most $n$ such women, and the number of previous proposals to such women is at least


\end{proof}

==> rwoman-concentration-sm.tex <==
	Within this proof, we assume that $\tau$, $\vec{W}_\tau = \left( W_{j,\tau} \right)_{j \in \mathcal{W}}$, and $\vec{W}_{(n+k)d} = \left( W_{j,(n+k)d} \right)_{j \in \mathcal{W}}$ are revealed (and hence so is $\bar{R}[\tau]$): In what follows, $\mathbb{P}( \cdot )$ and $\mathbb{E}[ \cdot ]$ denote the associated conditional probability and the conditional expectation, respectively.
	
	For brevity, let $w_j \triangleq W_{j,\tau}$, $w_j' \triangleq W_{j,(n+k)d} - W_{j,\tau}$, and $R_j \triangleq \text{Rank}_j( \text{MOSM}(j) )$. %\yk{What is the definition of $R_j$ if woman $j$ is unmatched? It should be degree + 1 if you want the average of $R_j$s to equal $\Rwomen$, right?}
	Note that a woman $j$ receives $w_j$ proposals until time $\tau$ and receives $w_j'$ proposals after time $\tau$ (the total number of proposals $w_j + w_j' = W_{j,(n+k)d}$ equals to her degree).
	Under MOSM, each woman $j$ is matched to her most preferred one among the first $w_j$ proposals, and the rank of her matched partner under MOSM, $R_j$, can be determined by the number of future proposals that she prefers to the matched partner among the remaining $w_j'$ proposals.
	
	
\edit{
	More specifically, fix $j$ and let $Y^j_{s,t}$ be the indicator that the woman $j$ prefers her $t^\text{th}$ proposal to her $s^\text{th}$ proposal for $s, t \in \{1, \ldots, w_j+w_j'\}$ with $s \ne t$.
	Then, the rank $R_j$ can be represented as
	\begin{align*}
		R_j &= 1 + \sum_{t=w_j+1}^{w_j+w_j'} \ind\left( \text{woman $j$ prefers her $t^\text{th}$ proposal to all of her first $w_j$ proposals} \right) 
			\\&= 1 + \sum_{t=w_j+1}^{w_j+w_j'} \prod_{s=1}^{w_j} \ind\left( \text{woman $j$ prefers her $t^\text{th}$ proposal to her $s^\text{th}$ proposal} \right) 
			\\&= 1 + \sum_{t=w_j+1}^{w_j+w_j'} \prod_{s=1}^{w_j} Y^j_{s,t}, \,
	\end{align*}
	where we define $\prod_{s=1}^{w_j} \cdot = 1$ if $w_j = 0$ for convenience.
	Observe that $\{ Y^j_{s,t} \}_{s,t}$ are negatively associated (NA) by Lemma \ref{lem:NA}-\eqref{lem:NA-permutation} since  $( Y^j_{s,t} )_{s,t \in \{1, \ldots, w_j+w_j'\}, s \ne t }$ is a uniformly random permutation of $\frac{ (w_j+w_j')(w_j+w_j'-1) }{2}$ ones and $\frac{ (w_j+w_j')(w_j+w_j'-1) }{2}$ zeros due to symmetry.
	\sm{May not be true}
	Consequently, $\prod_{s=1}^{w_j} Y^j_{s,t}$ is a component-wise increasing function of $Y^j_{1,t}, \ldots, Y^j_{w_j,t}$ and hence $\{ \prod_{s=1}^{w_j} Y^j_{s,t} \}_{t \in \{w_j+1, \ldots, w_j+w_j'\}}$ are also NA by Lemma \ref{lem:NA}-\eqref{lem:NA-monotone}.
	Also note that $\prod_{s=1}^{w_j} Y^j_{s,t} \sim \text{Bernoulli}\left( \frac{1}{w_j+1} \right)$ for each $t$.
	Therefore,
	\begin{equation*}
		\mathbb{E}\left[ R_j \right] = 1 + \frac{w_j'}{w_j+1},
	\end{equation*}
	and, for any $\lambda \in \mathbb{R}$, we have
	\begin{align*}
		\mathbb{E}\left[ \exp\left( \lambda (R_j-1) \right) \right]
			&\leq \prod_{t=w_j}^{w_j + w_j'} \mathbb{E}\left[ \exp\left( \lambda \prod_{s=1}^{w_j} Y^j_{s,t} \right) \right]
			= \left( 1 - \frac{1}{w_j+1} + \frac{1}{w_j+1} e^\lambda \right)^{w_j'}
			\\&\leq \exp\left( \frac{1}{w_j+1} \left(e^\lambda -1\right) \right)^{w_j'}
			= \exp\left( \frac{w_j'}{w_j+1} \left(e^\lambda -1\right) \right),
	\end{align*}
	where we utilized the fact that $\left\{ \exp\left( \lambda \prod_{s=1}^{w_j} Y^j_{s,t} \right) \right\}_{t \in \{w_j+1, \ldots, w_j+w_j'\}}$ are NA and that $1-x \leq e^{-x}$ for any $x \in \mathbb{R}$.
}
	
\edit{
	Further observe that $R_j$'s are independent across $j$ (conditioned on $\vec{W}_\tau$ and $\vec{W}_{(n+k)d}$).
	Therefore, for any $\lambda \in \mathbb{R}$, we obtain
	\begin{align*}
		\mathbb{E}\left[ \exp\left( \lambda \sum_{j \in \mathcal{W}} (R_j - 1) \right) \right]
			&= \prod_{j \in \mathcal{W}} \mathbb{E}\left[ \exp\left( \lambda (R_j-1) \right) \right]
			\leq \prod_{j \in \mathcal{W}} \exp\left( \frac{w_j'}{w_j+1} \left( e^\lambda -1 \right) \right)
			\\&= \exp\left( \sum_{j \in \mathcal{W}} \frac{w_j'}{w_j+1} \left( e^\lambda -1 \right) \right) 
			= \exp\left( n \bar{R}[\tau] (e^\lambda-1) \right),
	\end{align*}
	since $\bar{R}[\tau] = \frac{1}{n} \sum_{j \in \mathcal{W}} \frac{w_j'}{w_j+1}$ by its definition.
}

	\begin{equation*}
		R_j = 1 + \sum_{s=w_j+1}^{w_j+w_j'} X_{j,s}
	\end{equation*}
	where $X_{j,s}$ is defined as the indicator that woman $j$ prefers her $s^\text{th}$ incoming proposal (after termination of DA) to her partner under MOSM.
	Observe that $X_{j,s} \sim \text{Bernoulli}\left( \frac{1}{w_j+1} \right)$ and is independent across $j$ and $s$. \yk{I don't think it's independent! If the first three proposals are better than her partner, it becomes more likely her partner is shitty and hence the fourth proposal is more likely to also be better than her partner.. If you agree, then that breaks the claim it is Binomial below and stuff after that. However, I think you can nevertheless use Hoeffding's inequality to show that 
$$\mathbb{P}\left( \left. \Wrank \geq 1 + (1+\epsilon) \bar{R}[\tau] \,\right| \vec{W}_\tau, \vec{W}_{(n+k)d}\right) \leq 
\exp \left ( -\frac{2\eps^2  \bar{R}[\tau]^2 n^2 }{\sum_{j \in \mathcal{W}}W_{j,(n+k)d}^2 } \right )
$$. This should suffice since (i) you already showed that wvhp $\bar{R}[\tau] \geq \sqrt{d}/2$ and (ii) you can also show, using negative association that $\sum_{j \in \mathcal{W}}W_{j,(n+k)d}^2 / n$ is no more than $2d^2$ wvhp. Overall, the RHS should be less than $\exp(-n^{1-\epsilon})$ wvhp, which should suffice for your purposes, no?
} \edit{It follows from $X_{j,s} \sim \text{Bernoulli}\left( \frac{1}{w_j+1} \right)$ that the conditional expectation of $R_j = 1+ \frac{w_j'}{w_j+1}$ and hence that the conditional expectation of $\Wrank$ is $1+\bar{R}[\tau]$, which proves the first sentence of the lemma.}
	Therefore,
	\begin{equation*}
		-1 + R_j \stackrel{\text{d}}{=} \text{Binomial}\left( w_j', \frac{1}{w_j+1} \right),
	\end{equation*}
	and $R_j$'s are independent across $j$. \yk{I agree that $R_j$'s are independent across $j$.}
	Consequently, for any $\lambda \in \mathbb{R}$,
	\begin{align*}
		\mathbb{E}\left[ \exp\left( \lambda \sum_{j \in \mathcal{W}} (R_j - 1) \right) \right]
			&= \prod_{j \in \mathcal{W}} \left( 1 - \frac{1}{w_j+1} + \frac{1}{w_j+1} e^\lambda \right)^{w_j'}
			\leq \prod_{j \in \mathcal{W}} \exp\left( \frac{1}{w_j+1} (e^\lambda-1) \right)^{w_j'}
			\\&= \prod_{j \in \mathcal{W}} \exp\left( \frac{w_j'}{w_j+1} (e^\lambda-1) \right)
			= \exp\left( n \bar{R}[\tau] (e^\lambda-1) \right),
	\end{align*}
	since $\bar{R}[\tau] = \frac{1}{n} \sum_{j \in \mathcal{W}} \frac{w_j'}{w_j+1}$ by its definition.


	By Markov's inequality, for any $\lambda \in [0,1]$,
	\begin{align*}
		\mathbb{P}\left( -1 + \frac{1}{n} \sum_{j \in \mathcal{W}} R_j \geq (1+\epsilon) \bar{R}[\tau] \right)
			&\leq \frac{ \mathbb{E}\left[ \exp\left( \lambda \sum_{j \in \mathcal{W}} (R_j-1) \right) \right] }{ \exp\left( n \bar{R}[\tau] \lambda(1+\epsilon)  \right) }
			\\&\leq \exp\left(  n \bar{R}[\tau] (e^\lambda-1) - n \bar{R}[\tau] \lambda (1+\epsilon)   \right)
			\\&\leq \exp\left(  n \bar{R}[\tau] (\lambda + \lambda^2) - n \bar{R}[\tau] \lambda (1+\epsilon)   \right)
			= \exp\left( n \bar{R}[\tau] (\lambda^2 - \lambda \epsilon) \right),
	\end{align*}
	where we use the fact that $e^x \leq 1 + x + x^2$ for $x \leq 1$.
	By setting $\lambda \triangleq \frac{\epsilon}{2}$, we obtain
	\begin{align*}
		\mathbb{P}\left( \frac{1}{n} \sum_{j \in \mathcal{W}} R_j \geq 1 + (1+\epsilon) \bar{R}[\tau] \right) \leq \exp\left( - \frac{1}{4} \epsilon^2 n \bar{R}[\tau] \right).
	\end{align*}

